Immersed curves in Khovanov homology

We give a geometric interpretation of Bar-Natan's universal invariant for the class of tangles in the 3-ball with four ends: we associate with such 4-ended tangles $T$ multicurves $\widetilde{\operatorname{BN}}(T)$, that is, collections of immersed curves with local systems in the 4-punctured sphere. These multicurves are tangle invariants up to homotopy of the underlying curves and equivalence of the local systems. They satisfy a gluing theorem which recovers the reduced Bar-Natan homology of links in terms of wrapped Lagrangian Floer theory. Furthermore, we use $\widetilde{\operatorname{BN}}(T)$ to define two immersed curve invariants $\widetilde{\operatorname{Kh}}(T)$ and $\operatorname{Kh}(T)$, which satisfy similar gluing theorems that recover reduced and unreduced Khovanov homology of links, respectively. As a first application, we prove that Conway mutation preserves reduced Bar-Natan homology over the field with two elements and Rasmussen's $s$-invariant over any field. As a second application, we give a geometric interpretation of Rozansky's categorification of the two-stranded Jones-Wenzl projector. This allows us to define a module structure on reduced Bar-Natan and Khovanov homologies of infinitely twisted knots, generalizing a result by Benheddi.

==> PSTricks/sources/KhCurves-pics-header.tex <==
\usepackage[top=1in, bottom=1.25in, marginparwidth=1in, inner=1in, outer=1in]{geometry}

\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\renewcommand{\familydefault}{\ttdefault}

\usepackage{fancyheadings}

\pagestyle{empty}

\usepackage{graphicx}
\usepackage{xcolor}
\colorlet{myblue}{black}
\colorlet{gold}{yellow!90!black!70!red}
\colorlet{darkgreen}{green!70!black}
\colorlet{lightred}{red!30!white}
\colorlet{lightblue}{blue!30!white}

\usepackage{pstricks,pstricks-add}
\usepackage[crop=off,runs=1]{auto-pst-pdf}
\usepackage{pst-plot}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}

\newcommand{\m}{\operatorname{m}}% old mirror command
\input{../../notation_commands.tex}

% predefined functions for morphism classification

\newcommand{\dotcircle}{\pscircle[linestyle=dotted,dotsep=1pt](0,0){2}}
\newcommand{\cobcircle}{\pscircle[linewidth=0.25pt](0,0){2}}

\makeatletter
\def\bpt{\pst@object{bpt}}
\def\bpt@i#1(#2){%
	\begin@OpenObj%
	\psdot[dotstyle=asterisk,dotsize=4pt,dotangle=#1](#2)
	\psdot[dotsize=0.8pt](#2)
	\end@OpenObj%
}
\def\pswrap{\pst@object{pswrap}}
\def\pswrap@i#1(#2)#3{%
	\begin@OpenObj%
	\rput{#3}(0,0){%
		\parametricplot[#1,plotstyle=curve,plotpoints=300,algebraic]{0}{#2}%
		{10*(1-(t/5)^(1/2)/2)*cos(2*Pi*t/4)|10*(1-(t/5)^(1/2)/2)*sin(2*Pi*t/4)}%
	}
	\end@OpenObj%
}
\def\pswrapn{\pst@object{pswrapn}}
\def\pswrapn@i#1(#2)#3{%
	\begin@OpenObj%
	\rput{#3}(0,0){%
		\parametricplot[#1,plotstyle=curve,plotpoints=300,algebraic]{0}{#2}%
		{10*(1-((#2-t)/5)^(1/2)/2)*cos(2*Pi*(#2-t)/4)|10*(1-((#2-t)/5)^(1/2)/2)*sin(2*Pi*(#2-t)/4)}%
	}
	\end@OpenObj%
}
\def\pswrapend{\pst@object{pswrapend}}
\def\pswrapend@i#1(#2)#3{%
	\begin@ClosedObj%
	\rput{#3}(0,0){%
		\psline[arrows=->,#1]%
		(!10 1 #2 5 div 1 2 div exp 2 div sub mul 360 #2 mul 4 div cos mul 10 1 #2 5 div 1 2 div exp 2 div sub mul 360 #2 mul 4 div sin mul)(!10 360 #2 mul 4 div cos mul 10 360 #2 mul 4 div sin mul)
	}
	\end@ClosedObj%
}
\def\psMorBoundary{\pst@object{psMorBoundary}}
\def\psMorBoundary@i#1{%
	\begin@ClosedObj%
	\rput*{#1}(0,0){
		\pscustom*[linecolor=lightred,linewidth=0pt]{
			\psarc(0,0){10}{-20}{20}
			\psline(10;20)(12;20)
			\psarcn(0,0){12}{20}{-20}
			\psline(12;-20)(10;-20)
		}
		\psarc(0,0){10}{-20}{20}
		\psline(9.7;0)(10.3;0)
	}
	\end@ClosedObj%
}
\def\psLagwrap{\pst@object{psLagwrap}}
\def\psLagwrap@i#1#2(#3)#4#5{%
	% #1 is a scalar, usually 0.5, which is the maximal radius 
	% #2 is an angle, which rotates the picture
	% #3 is a coordinate x,y
	% #4 is a colour
	% #5 is a number and defined the start of the curve (usually 0)
	\begin@ClosedObj%
	\rput{#2}(#3){
		\parametricplot[linecolor=#4,plotstyle=curve,plotpoints=200]{#5}{10}{%
			0.14 #1 0.14 sub 1 t t mul add div add 360 t mul cos mul
			0.14 #1 0.14 sub 1 t t mul add div add 360 t mul sin mul
		}}
	\end@ClosedObj%
}
\def\psLi{%
	\psrotate(0,0){45}{
		\dotcircle
		%\psdot[linecolor=red](0,2)
		\rput(0,2){$\ast$}
		\pscustom{
			\psline(0,2)(0,1)
			\psarcn(-1,1){1}{0}{-90}
			\psline(-1,0)(-2,0)
		}%
		\pscustom{
			\psline(0,-2)(0,-1)
			\psarcn(1,-1){1}{180}{90}
			\psline(1,0)(2,0)
		}%
	}
}
\def\psLo{%
	\psrotate(0,0){45}{
		\dotcircle
		%\psdot[linecolor=red](0,2)
		\rput(0,2){$\ast$}
		\pscustom{
			\psline(0,2)(0,1)
			\psarc(1,1){1}{-180}{-90}
			\psline(1,0)(2,0)
		}%
		\pscustom{
			\psline(0,-2)(0,-1)
			\psarc(-1,-1){1}{0}{90}
			\psline(-1,0)(-2,0)
		}%
	}
}	
\makeatother



\newlength{\stringwidth}
\setlength{\stringwidth}{1.5pt}
\newlength{\stringwhite}
\setlength{\stringwhite}{5.5pt}

\newlength{\stringwidthThick}
\setlength{\stringwidthThick}{2.5pt}
\newlength{\stringwhiteThick}
\setlength{\stringwhiteThick}{7.5pt}


